Unlocking the Potential of Text-to-Image Diffusion with PAC-Bayesian Theory

Text-to-image (T2I) diffusion models have revolutionized generative modeling by producing high-fidelity, diverse, and visually realistic images from textual prompts. Despite these advances, existing models struggle with complex prompts involving multiple objects and attributes, often misaligning modifiers with their corresponding nouns or neglecting certain elements. Recent attention-based methods have improved object inclusion and linguistic binding, but still face challenges such as attribute misbinding and a lack of robust generalization guarantees. Leveraging the PAC-Bayes framework, we propose a Bayesian approach that designs custom priors over attention distributions to enforce desirable properties, including divergence between objects, alignment between modifiers and their corresponding nouns, minimal attention to irrelevant tokens, and regularization for better generalization. Our approach treats the attention mechanism as an interpretable component, enabling fine-grained control and improved attribute-object alignment. We demonstrate the effectiveness of our method on standard benchmarks, achieving state-of-the-art results across multiple metrics. By integrating custom priors into the denoising process, our method enhances image quality and addresses long-standing challenges in T2I diffusion models, paving the way for more reliable and interpretable generative models.

==> sec/0_pre.tex <==
%3. 4.3.1 往前放，我们希望attation map 有哪些特点。 试了很多不同的prior，选了4个。 User should design their own prior，只不过我们做了这样的，其他人也可以这样做，突出bayesion framework novelity

%5. Method 先讲problem formulation。不要加一些新的notation。 Problem: prompt -> token (4.2.1)
%6. Better loss name for outside loss.

\section{Introduction} \label{sec
}

Text-to-image diffusion models have revolutionized the field of generative modeling, enabling the creation of high-fidelity images conditioned on textual descriptions~\cite{Rombach22,Nichol21,Saharia22,Ho20,Dhariwal21,Song21,Kingma21}. These models have demonstrated remarkable capabilities in generating diverse and realistic images, pushing the boundaries of creativity and visual representation~\cite{Radford21,Esser21,Dosovitskiy21,Brock19,Goodfellow14,Reed2016generative}. Techniques like classifier-free guidance~\cite{Ho2022classifier} and improved training strategies~\cite{Nichol2021improved} have further enhanced their performance. Despite their impressive achievements, these models often face challenges when handling complex prompts containing multiple objects and attributes~\cite{Zhang24,Chefer23,Feng23,Liu22,Rassin23}. Specifically, they may struggle with correctly associating modifiers to the appropriate nouns and allocating balanced attention among different elements in the prompt, leading to images that do not accurately reflect the intended description~\cite{Rassin23,Chefer23,Zhang24, chang2024skews, zhang2024objectconditioned}.

The problem of attribute misbinding and object neglect in text-to-image generation has been extensively studied~\cite{Zhang24,Rassin23,Chefer23,Zhang2023adding,Park23,Agarwal23}. For instance, Zhang et al.\cite{Zhang24} observed that diffusion models may generate images with incorrect attribute bindings or completely neglect certain objects mentioned in the prompt. Similarly, Chefer et al.\cite{Chefer23} introduced the \emph{Attend-and-Excite} method to enhance object presence but noted that it may lead to attribute leakage and artifacts. Rassin et al.\cite{Rassin23} highlighted the limitations of existing attention mechanisms in correctly capturing attribute-object relationships. Moreover, issues such as object hallucination\cite{Kim2022diffusionclip}, semantic confusion~\cite{Gal2022an}, and context misalignment~\cite{Li2023gligen} further exacerbate these challenges.

A significant part of this challenge stems from the attention mechanisms within these models, which often function as black boxes~\cite{Esser21,Rassin23,Feng23,Hertz23,Vaswani17}. The lack of transparency and control over attention distributions makes it difficult to guide the model towards desired behaviors, such as correct attribute binding and balanced attention allocation~\cite{Hertz23,Avrahami2022blended,Brooks2023instructpix2pix}. Without a way to influence the attention maps, users have limited ability to correct misalignments between the textual input and the generated images~\cite{Hertz23,Chefer23,Rassin23}.

Several approaches have been proposed to address these issues. Hertz et al.\cite{Hertz23} introduced \emph{Prompt-to-Prompt} editing, allowing users to control the generation process by manipulating cross-attention maps. Liu et al.\cite{Liu22} proposed \emph{Composable Diffusion} models that compose multiple outputs guided by different objects in the text prompt. Feng et al.\cite{Feng23} presented \emph{Training-Free Structured Diffusion Guidance} to enhance compositionality in text-to-image synthesis. However, these methods may still suffer from attribute misbinding and lack theoretical guarantees on their generalization performance\cite{Zhang24,Chefer23}.

Recently, Zhang et al.\cite{Zhang24} introduced an \emph{Object-Conditioned Energy-Based Attention Map Alignment} (EBAMA) method to address attribute binding and object neglect problems. Their approach leverages an energy-based model to align attention maps between attributes and objects, improving semantic alignment. While effective, their method focuses on specific energy functions and may not provide a flexible framework for designing custom attention priors\cite{Park23}. Additionally, methods like \emph{A-STAR}\cite{Agarwal23} and \emph{GLIGEN}\cite{Li2023gligen} have attempted to incorporate external knowledge or grounding mechanisms but may introduce additional complexity.

In this paper, we propose a novel Bayesian framework to guide the attention mechanisms in text-to-image diffusion models. By formalizing the problem within the PAC-Bayes framework~\cite{McAllester99}, we provide a principled approach that allows users to design their own priors over attention distributions, specifying desirable characteristics for the attention maps. We experimented with various priors and selected key components that enforce attention map properties such as divergence between different objects, similarity between modifiers and their corresponding nouns, minimal attention to irrelevant tokens, and regularization to prevent overfitting.

Our approach differs from previous works in that it treats the attention mechanism not as a black box, but as an interpretable component that can be guided using Bayesian principles. By minimizing the Kullback-Leibler divergence between the learned attention distributions and the designed priors, we effectively guide the model to produce images with better attribute-object alignment and balanced attention allocation. Importantly, this framework is flexible, allowing users to define their own priors based on specific needs or preferences, thereby highlighting the novelty and versatility of our Bayesian approach.

Our contributions can be summarized as follows:

\begin{itemize} \item We introduce a novel Bayesian framework that allows for the design of custom priors over attention distributions in text-to-image diffusion models, enhancing control over the attention mechanism and addressing the black-box nature of existing models. \item We formalize the problem within the PAC-Bayes framework~\cite{McAllester99}, providing theoretical guarantees on the generalization performance and highlighting the novelty of our approach. \item We demonstrate that our method achieves state-of-the-art results on standard benchmarks~\cite{Chefer23, Feng23, Rassin23}, improving attribute binding accuracy and attention allocation in generated images, thus validating the effectiveness of our framework. \end{itemize}

\section{Related Works}

\subsection{Stable Diffusion}

Stable Diffusion~\cite{Rombach22} is a seminal work in text-to-image synthesis that employs a latent diffusion model to generate high-resolution images efficiently. By operating in a lower-dimensional latent space \cite{yu2024latent} learned through an autoencoder~\cite{Esser21,Rombach21}, Stable Diffusion significantly reduces computational requirements compared to pixel-space diffusion models~\cite{Sohl-Dickstein2015deep,Ho20,Dhariwal21}. It leverages cross-attention mechanisms~\cite{Vaswani17,Parmar2018image} to align textual and visual information, enabling the generation of diverse and detailed images conditioned on textual prompts~\cite{Nichol21,Saharia22, Li2023}. Techniques such as classifier-free guidance~\cite{Ho2022classifier} and improved training objectives~\cite{Nichol2021improved} have further enhanced the quality and controllability of generated images \cite{zhang2024flow, zhu2024think}. However, despite its success, Stable Diffusion and similar models often struggle with complex prompts involving multiple objects and attributes~\cite{Rassin23,Chefer23,Feng23}, leading to issues such as attribute misbinding and object neglect.

\subsection{Bayesian Learning and PAC-Bayes Framework}

The PAC-Bayes framework~\cite{McAllester99} provides theoretical tools for analyzing the generalization performance of learning algorithms, especially those involving stochastic predictors \cite{zhang2024statistical}. By incorporating prior knowledge in the form of a prior distribution over hypotheses, PAC-Bayes offers generalization bounds that can guide model selection and regularization. Bayesian methods have been applied to various domains in machine learning, including neural networks and attention mechanisms~\cite{Ho2022classifier,Meng2021sdedit}, offering a principled way to incorporate uncertainty and prior information. In the context of diffusion models, Bayesian approaches have been used to improve image restoration~\cite{Kawar2022denoising} and editing~\cite{Avrahami2022blended}. In our work, we adopt the PAC-Bayes framework to design custom priors over attention distributions in diffusion models, enabling controlled and interpretable attention mechanisms that improve attribute-object alignment.

%-------------------------------------------------------------------------
\begin{figure}[h]
    \centering
    \includegraphics[width=0.475\textwidth]{photo/flow_1.png}
    \caption{\textbf{An overview of our workflow for optimizing the stable diffusion model.} It includes aggregation of attention maps, computation of object-centric attention loss, and updates to $z_t$.}
    \label{fig:flow_image}
\end{figure}

\section{Background}
\label{sec:background}

\subsection{Stable Diffusion Models}

Stable Diffusion Models (SD)~\cite{Rombach22}. SD first encodes an image \( x \) into the latent space using a pretrained encoder~\cite{Esser21}, i.e., \( z = E(x) \). Given a text prompt \( y \), SD optimizes the conditional denoising autoencoder \( \epsilon_\theta \) by minimizing the objective:

\begin{equation}
\mathcal{L}_\theta = \mathbb{E}_{t, \epsilon \sim \mathcal{N}(0,1), z \sim \mathcal{E}(x)} \left\| \epsilon - \epsilon_\theta(z_t, t, \phi(y)) \right\|^2,
\label{eq:sd_loss}
\end{equation}

where \( \phi \) is a frozen CLIP text encoder~\cite{Radford21}, \( z_t \) is a noised version of the latent \( z \), and the time step \( t \) is uniformly sampled from \( \{1, \dots, T\} \). During sampling, \( z_T \) is randomly sampled from standard Gaussian and denoised iteratively by the denoising autoencoder \( \epsilon_\theta \) from time \( T \) to \( 0 \). Finally, a decoder \( D \) reconstructs the image as \( \tilde{x} = D(z_0) \).

\subsection{Cross-Attention Mechanism}

In the cross-attention mechanism, \( K \) is the linear projection of \( W_y \), the CLIP-encoded text embeddings of text prompt \( y \). \( Q \) is the linear projection of the intermediate image representation parameterized by latent variables \( z \). Given a set of queries \( Q \) and keys \( K \), the (unnormalized) attention features and (softmax-normalized) scores between these two matrices are:

\begin{equation}
A = \frac{Q K^\top}{\sqrt{m}}, \quad \tilde{A} = \text{softmax} \left( \frac{Q K^\top}{\sqrt{m}} \right),
\label{equ:attn}
\end{equation}

where \( m \) is the feature dimension. We consider both attention features and scores for our modeling here, which we denote as \( A_s \) and \( \tilde{A}_s \) for token \( s \), respectively.

%-------------------------------------------------------------------------

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{photo/photo_3.png}
    \caption{\textbf{Qualitative comparison on the ABC-6K dataset.} We compared our model using the same prompt and random seed as SD \cite{Rombach21}, SG \cite{Rassin23}, AnE \cite{Chefer23}, and EMAMA \cite{Zhang24}, with each column sharing the same random seed.}
    \label{fig:body_image}
\end{figure*}

\section{Method and Theoretical Foundations}
\label{sec:method}

In this section, we introduce our method designed to guide the attention mechanism of text-to-image diffusion models when processing prompts containing multiple objects. Our approach leverages the attention maps produced by the model to ensure balanced attention, correct attribute association, and improved generalization.

\subsection{Attention Map Distribution}

We focus on the extraction of nouns and modifiers from the text prompt and how the model can find their interactions. For example, given a prompt like \emph{`a frog and a purple crown''}, we use a natural language parser to identify the nouns (\emph{frog''}, \emph{crown''}) and modifiers (\emph{purple''}), and determine the associations between them.

By analyzing the syntactic structure of the prompt, the parser can identify that \emph{`purple''} modifies \emph{crown''}, and not \emph{frog''}. This information is crucial for guiding the attention mechanism so that the model correctly associates attributes with the corresponding objects in the generated image.

Our method involves mapping the tokens in the prompt to their corresponding attention maps. By aligning the attention maps with the syntactic structure of the prompt, we can enforce constraints that encourage the model to attend appropriately to different parts of the image during generation.

\subsection{PAC-Bayes Framework}

To formalize our approach, we employ the PAC-Bayes framework~\cite{}, which provides a theoretical foundation for understanding the generalization properties of learning algorithms.

\begin{definition}[PAC-Bayes Bound]
Given a prior distribution \( P \) over hypotheses \( h \in \mathcal{H} \), with probability at least \( 1 - \delta \), the following inequality holds:

\begin{equation}
\begin{aligned}
\mathbb{E}_{h \sim Q} [\text{Risk}(h)] &\leq \mathbb{E}_{h \sim Q} [\widehat{\text{Risk}}(h)] + \\
&\quad \sqrt{ \frac{ D_{\text{KL}}(Q \parallel P) + \ln \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
\end{aligned}
\label{eq:pac_bayes_bound}
\end{equation}

where \( Q \) is the posterior distribution over hypotheses, \( \text{Risk}(h) \) is the true risk, \( \widehat{\text{Risk}}(h) \) is the empirical risk, \( D_{\text{KL}}(Q \parallel P) \) is the Kullback-Leibler divergence between \( Q \) and \( P \), \( N \) is the number of samples, and \( \delta \) is the confidence parameter (\( 0 < \delta < 1 \)).
\end{definition}

%\subsubsection{Why PAC-Bayes?}
The PAC-Bayes framework allows us to derive generalization bounds that depend on the divergence between the learned model and a prior belief. By incorporating prior knowledge about how attention should be distributed in the model (e.g., modifiers should be associated with their corresponding nouns), we can guide the learning process in a principled way.

Minimizing the KL divergence \( D_{\text{KL}}(Q \parallel P) \) ensures that the learned attention distributions \( Q \) are close to the prior \( P \), which encodes our desired properties. This helps to prevent overfitting and improves the generalization performance of the model.

\subsubsection{Representation of Attention Maps}

% We model the attention maps 
% as probability distributions 
% over a finite set \( \Omega \) (e.g., spatial locations in the image). Specifically, we represent each attention map \( A_i \) as a flattened vector of dimension \( n \times 1 \), where \( n \) is the number of elements (e.g., \( 16 \times 16 = 256 \) for a \( 16 \times 16 \) attention map). Each element \( A_i(j) \) satisfies:
% \begin{equation}
% A_i(j) \geq 0 \forall j \in \Omega; \quad \sum_{j \in \Omega} A_i(j) = 1,
% \label{eq:attention_distribution}
% \end{equation} 

We model the attention maps 
as probability distributions
over a finite set \( \Omega \), where \( \Omega \) denotes the spatial indices within the image. 
 Each entry \( A_i(j) \) represents a non-negative weight at spatial location $j$, satisfies:
\begin{equation}
A_i(j) \geq 0 \quad \forall j \in \Omega; \quad \sum_{j \in \Omega} A_i(j) = 1,
\label{eq:attention_distribution}
\end{equation} 

This ensures that the attention maps are valid probability distributions (i.e., multinomial distributions), facilitating the use of information-theoretic measures like the KL divergence.

% We represent each attention map \( A_i \) as a flattened vector of dimension \( n \times 1 \), where \( n \) is the number of elements (e.g., \( 16 \times 16 = 256 \) for a \( 16 \times 16 \) attention map). 

\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{photo/photo_4.png}
    \caption{\textbf{Qualitative comparison on the AnE dataset (left two columns) and the DVMP dataset.} We compared our model using the same prompt and random seed as SD \cite{Rombach21}, SG \cite{Rassin23}, AnE \cite{Chefer23}, and EMAMA \cite{Zhang24}, with each column sharing the same random seed.}

    \label{fig:body_image}
\end{figure*}


\subsection{Our Algorithm}

From the PAC-Bayes inequality in Equation~\eqref{eq:pac_bayes_bound}, we aim to minimize the KL divergence \( D_{\text{KL}}(Q \parallel P) \) between the posterior \( Q \) and the prior \( P \), while keeping \( N \) and \( \delta \) constant.

\subsubsection{Prior and Posterior Distributions}

We define the prior distribution \( P(A) \) over attention maps \( A \) as a human-designed distribution that encodes our desired properties. Specifically, we factorize \( P(A) \) as:

\begin{equation}
P(A) \propto \left( P_1(A) \right)^\alpha \left( P_2(A) \right)^\beta \left( P_3(A) \right)^\gamma \left( P_4(A) \right)^\eta,
\label{eq:prior_factorization}
\end{equation}

where:

\begin{itemize}
    \item \( P_1(A) \) corresponds to the divergence component, encouraging the attention maps of different objects to be separated.
    \item \( P_2(A) \) corresponds to the similarity component, encouraging modifiers and their associated nouns to have similar attention maps.
    \item \( P_3(A) \) corresponds to the outside component, discouraging attention to irrelevant tokens (e.g., articles like \emph{`a''}, \emph{the''}).
    \item \( P_4(A) \) corresponds to the regularizer, promoting generalization and preventing overfitting.
\end{itemize}

The exponents \( \alpha, \beta, \gamma, \eta \) are nonnegative hyperparameters controlling the influence of each component, satisfying \( \alpha + \beta + \gamma + \eta = 1 \).

The prior \( P(A) \) is designed to capture our prior beliefs about the attention distributions. The likelihood \( P(B | A) \) models the probability of observing the data \( B \) (e.g., the latent variables \( z_t \)) given the attention maps \( A \). The posterior \( Q(A) \) represents the learned attention distributions given the data.

\subsubsection{Minimizing Q and P}


Our goal is to minimize the KL divergence between the posterior and the prior:

\begin{equation}
D_{\text{KL}}(Q \parallel P) = \sum_{A} Q(A) \log \left( \frac{Q(A)}{P(A)} \right).
\label{eq:kl_divergence_qp}
\end{equation}

Substituting the factorized prior \( P(A) \) from Equation~\eqref{eq:prior_factorization}, we have:
\begin{equation}
\begin{aligned}
D_{\text{KL}}(Q \parallel P) &= \sum_{A} Q(A) \log \bigg( \frac{Q(A)}{\frac{1}{Z} \left( P_1(A) \right)^\alpha \left( P_2(A) \right)^\beta}  \\
&\quad  \times \left( P_3(A) \right)^\gamma \left( P_4(A) \right)^\eta \bigg) 
\end{aligned}
\end{equation}


% { \footnotesize
% \begin{align}
% D_{\text{KL}}(Q \parallel P) &= \sum_{A} Q(A) \log \left( \frac{Q(A)}{\frac{1}{Z} \left( P_1(A) \right)^\alpha \left( P_2(A) \right)^\beta \left( P_3(A) \right)^\gamma \left( P_4(A) \right)^\eta} \right) \nonumber \\
% &= \sum_{A} Q(A) \log Q(A) \nonumber \\
% &\quad - \sum_{A} Q(A) \left( \alpha \log P_1(A) + \beta \log P_2(A) \right. \nonumber \\
% &\qquad \left. + \gamma \log P_3(A) + \eta \log P_4(A) - \log Z \right),
% \end{align}
% }


where \( Z \) is the normalization constant. Since \( \log Z \) is a constant, we can omit it during optimization, resulting in: 

% The KL divergence then becomes:

% { \footnotesize
% \begin{align*}
% D_{\text{KL}}(Q \parallel P) &= \sum_{A} Q(A) \log Q(A) - \alpha \sum_{A} Q(A) \log P_1(A) \\
% &\quad - \beta \sum_{A} Q(A) \log P_2(A) \\
% &\quad - \gamma \sum_{A} Q(A) \log P_3(A) - \eta \sum_{A} Q(A) \log P_4(A) + \text{Constant}.
% \end{align*}
% }


% This can be rewritten as:
{ \footnotesize
\begin{equation}
\begin{aligned}
D_{\text{KL}}(Q \parallel P) &= \alpha \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_1(A)} \right) + \beta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_2(A)} \right) \\
&\quad + \gamma \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_3(A)} \right) + \eta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_4(A)} \right) \\
&\quad + \left( 1 - \alpha - \beta - \gamma - \eta \right) \sum_{A} Q(A) \log Q(A) + \text{const}.
\end{aligned}
\end{equation}
}
% { \footnotesize
% \begin{align}
% D_{\text{KL}}(Q \parallel P) &= \alpha \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_1(A)} \right) + \beta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_2(A)} \right) \nonumber \\
% &\quad + \gamma \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_3(A)} \right) + \eta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_4(A)} \right)\\
% & + \left( 1 - \alpha - \beta - \gamma - \eta \right) \sum_{A} Q(A) \log Q(A) + \text{const}.
% \end{align}
% }



Therefore, minimizing \( D_{\text{KL}}(Q \parallel P) \) is equivalent to minimizing the weighted sum of KL divergences between \( Q(A) \) and each \( P_i(A) \) for $i = 1, \dots, 4$:

{ \footnotesize
\begin{align}
D_{\text{KL}}(Q \parallel P) &= \alpha D_{\text{KL}}(Q \parallel P_1) + \beta D_{\text{KL}}(Q \parallel P_2) \nonumber \\
&\quad + \gamma D_{\text{KL}}(Q \parallel P_3) + \eta D_{\text{KL}}(Q \parallel P_4) + \text{const}.
\end{align}
}

This brings us to our total loss function, which combines the four components: divergence, similarity, outside, and regularization losses.

\subsection{Final Loss Function}

The final loss function we optimize is:

\begin{equation}
\mathcal{L}_{\text{total}} = \lambda_{\text{div}} \mathcal{L}_{\text{div}} + \lambda_{\text{sim}} \mathcal{L}_{\text{sim}} + \lambda_{\text{out}} \mathcal{L}_{\text{out}} + \lambda_{\text{PAC}} \mathcal{R}_{\text{PAC}},
\label{eq:total_loss_final}
\end{equation}

where \( \lambda_{\text{div}} = \alpha \), \( \lambda_{\text{sim}} = \beta \), \( \lambda_{\text{out}} = \gamma \), and \( \lambda_{\text{PAC}} = \eta \), corresponding to the exponents in the prior distribution.

By minimizing this loss, we effectively minimize \( D_{\text{KL}}(Q \parallel P) \) and, according to the PAC-Bayes bound, control the generalization error of our model.

\subsubsection{Divergence Loss}

The divergence loss $\mathcal{L}_{\text{divergence}}$ measures the symmetric Kullback-Leibler (KL) divergence between the combined attention maps of the two objects in the prompt. This component encourages the model to allocate attention evenly between the objects.

Let $A_{\text{object1}}$ and $A_{\text{object2}}$ denote the combined attention maps for object 1 and object 2, respectively. The divergence loss is defined as:

\begin{equation}
\mathcal{L}_{\text{divergence}} = - \frac{1}{2} \left[ D_{\text{KL}}(A_{\text{obj1}} \parallel A_{\text{obj2}}) + D_{\text{KL}}(A_{\text{obj2}} \parallel A_{\text{obj1}}) \right]
\label{eq:divergence_loss}
\end{equation} % 这个是个负值，不是正的。

For this loss, we want the two objects to be away from each other. By doing the KL convergence away from the object(1) attention map to object(2). The model can distinguish the difference between the two objects.  

\subsection{Similarity Loss}

The similarity loss $\mathcal{L}_{\text{similarity}}$ promotes coherence within each object by encouraging the attention maps of modifiers and nouns to be similar.

For each object $k \in \{1, 2\}$:

\begin{itemize}
    \item Let $\mathcal{M}_k$ be the set of modifier indices (e.g., adjectives).
    \item Let $\mathcal{N}_k$ be the set of noun indices.
    \item Define the set of modifier-noun pairs $\mathcal{P}_k = \{ (i, j) \mid i \in \mathcal{M}_k, \, j \in \mathcal{N}_k \}$.
\end{itemize}

The similarity loss for object $k$ is:

\begin{equation}
\mathcal{L}_{\text{similarity}}^{(k)} = \frac{1}{|\mathcal{P}_k|} \sum_{(i, j) \in \mathcal{P}_k} D_{\text{sym}}(A_i, A_j)
\label{eq:similarity_loss_k}
\end{equation}

where $D_{\text{sym}}(A_i, A_j)$ is the symmetric KL divergence between attention maps $A_i$ and $A_j$:

\begin{equation}
D_{\text{sym}}(A_i, A_j) = \frac{1}{2} \left[ D_{\text{KL}}(A_i \parallel A_j) + D_{\text{KL}}(A_j \parallel A_i) \right]
\label{eq:symmetric_kl}
\end{equation}

The total similarity loss is the sum over both objects:

\begin{equation}
\mathcal{L}_{\text{similarity}} = \mathcal{L}_{\text{similarity}}^{(1)} + \mathcal{L}_{\text{similarity}}^{(2)}
\label{eq:similarity_loss}
\end{equation}

Here this loss, we want to maximize the attention map of modifiers using KL correspond to their attention map of the object. For example, a pink crown and a purple bow, we want the attention map of pink and attention map of crown to be similar to each other. %这里比较像 Linguistic blinding 那篇论文。



\subsection{Outside Loss}

The outside loss $\mathcal{L}_{\text{outside}}$ discourages the attention maps of object tokens from being similar to those of unrelated tokens (outside tokens).

Let:

\begin{itemize}
    \item $\mathcal{S} = \mathcal{M}_1 \cup \mathcal{N}_1 \cup \mathcal{M}_2 \cup \mathcal{N}_2$: The set of all object token indices.
    \item $\mathcal{O} = \text{All Indices} \setminus \mathcal{S}$: The set of outside token indices.
\end{itemize}

The outside loss is defined as:

\begin{equation}
\mathcal{L}_{\text{outside}} = -\frac{1}{|\mathcal{S}|} \sum_{i \in \mathcal{S}} \left( \max_{j \in \mathcal{O}} D_{\text{sym}}(A_i, A_j) \right)
\label{eq:outside_loss}
\end{equation}

This loss component prevents the model from confusing object-specific tokens with unrelated tokens. By penalizing high similarity between them, the model learns to focus on relevant parts of the prompt, improving the clarity and accuracy of the generated images. % 这个写的没问题 像Snygen 那篇文章

\subsection{PAC-Bayes Regularizer}

The PAC-Bayes regularizer $\mathcal{R}_{\text{PAC}}$ incorporates principles from PAC-Bayes theory to regularize the attention distributions, promoting generalization.

Let $N$ be the number of samples and $\delta$ be the confidence parameter. The regularizer is computed as:

\begin{equation}
\mathcal{R}_{\text{PAC}} = -\sqrt{ \frac{ \left( \dfrac{1}{2} \sum\limits_{k=1}^{2} D_{\text{KL}}(A_{\text{object}k} \parallel U) \right) + \log \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
\label{eq:pac_bayes_regularizer}
\end{equation} % 应该是负数，应该离 uniform distribution 越远越好 

Here, $U$ represents the uniform distribution over the attention map dimensions.

The goal of this formula is to make the attention map away from the uniform distribution. The PAC prevents the model from becoming overly confident in specific attention patterns, prevents overfitting. 

(1) The PAC-Bayes feeds the not uniform distribution into the model as the prior 






\begin{table*}[ht]
    \centering
    \label{tab:clip_scores}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|ccc|ccc|}
        \hline
        \textbf{Method} & \multicolumn{3}{c|}{\textbf{Animal-Animal}} & \multicolumn{3}{c|}{\textbf{Animal-Object}} & \multicolumn{3}{c|}{\textbf{Object-Object}} \\
        \hline
         & \textbf{Full Sim.} & \textbf{Min. Sim.} & \textbf{T-C Sim.} & \textbf{Full Sim.} & \textbf{Min. Sim.} & \textbf{T-C Sim.} & \textbf{Full Sim.} & \textbf{Min. Sim.} & \textbf{T-C Sim.} \\
        \hline
        SD \cite{Rombach22} & 0.311 & 0.213 & 0.767 & 0.340 & 0.246 & 0.793 & 0.335 & 0.235 & 0.765 \\
        CD \cite{Liu22} & 0.284 & 0.232 & 0.692 & 0.336 & 0.252 & 0.769 & 0.349 & 0.265 & 0.759 \\
        StrD \cite{Feng23} & 0.306 & 0.210 & 0.761 & 0.336 & 0.242 & 0.781 & 0.332 & 0.234 & 0.762 \\
        EBCA \cite{Park23} & 0.291 & 0.215 & 0.722 & 0.317 & 0.229 & 0.732 & 0.321 & 0.231 & 0.726 \\
        AnE \cite{Chefer23} & 0.332 & 0.248 & 0.806 & 0.353 & 0.265 & 0.830 & 0.360 & 0.270 & 0.811 \\
        SG \cite{Rassin23} & 0.311 & 0.213 & 0.767 & 0.355 & 0.264 & 0.830 & 0.355 & 0.262 & 0.811 \\
        EBAMA \cite{Zhang24} & 0.340 & 0.256 & 0.817 & 0.362 & 0.270 & 0.851 & 0.366 & 0.274 & 0.836 \\
        D\&B \cite{Li2023} & 0.331 & 0.246 & 0.810 & -- & -- & -- & -- & -- & -- \\
        \hline
        \textbf{Ours} & \textbf{0.348} & \textbf{0.262} & \textbf{0.823} & \textbf{0.370} & \textbf{0.276} & \textbf{0.868} & \textbf{0.370} & \textbf{0.275} & \textbf{0.844} \\
        \hline
    \end{tabular}
    }
    \caption{ \textbf{ Comparison of Full Sim., Min. Sim., and T-C Sim. across different methods on the AnE dataset. CLIP Score based on the Attend and Excite Dataset.} Note that the performance of SG on Animal-Animal is degraded to SD, as the prompts do not contain any attribute-object pairs. The best results for each category is marked in bold numbers.}

\end{table*}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.475\textwidth]{photo/photo_chart.png}
    \caption{ \textbf{Full Sim. results on DVMP and ABC-6K datasets.} We randomly sample 200 prompts from each dataset and generate 4 images for each prompt.}
    \label{fig:chart_image}
\end{figure}


\section{Workflow}

Our proposed method integrates custom attention priors into the denoising process of text-to-image diffusion models, specifically Stable Diffusion~\cite{Rombach22}. We begin by parsing the input prompt using a natural language parser to extract nouns and their associated modifiers, identifying the relationships between them. During each denoising step, we extract the cross-attention maps corresponding to these tokens. We then apply custom loss functions based on the Kullback-Leibler divergence between the learned attention distributions and our designed priors, guided by the PAC-Bayes framework~\cite{McAllester99}. This includes losses that encourage divergence between different objects' attention maps, similarity between modifiers and their nouns, minimal attention to irrelevant tokens, and a regularization term to prevent overfitting. By combining these losses, we update the latent representations iteratively, refining the generated image to better align with the input prompt and improving attribute binding accuracy.


Algorithm~\ref{alg:syngen_step} outlines a single denoising step using our proposed loss function.

\begin{algorithm}[H]
\caption{A Single Denoising Step using PAC}
\label{alg:syngen_step}
\begin{algorithmic}[1]
\Statex \textbf{Input:} Text prompt $P$, latents $\mathbf{z}_t$, text embeddings $\mathbf{E}$, timestep $t$, iteration $i$, step size $\alpha_t$, number of intervention steps $K$, trained Stable Diffusion model $\text{SD}$, loss hyperparameters $\lambda_{\text{div}}$, $\lambda_{\text{sim}}$, $\lambda_{\text{out}}$, $\lambda_{\text{PAC}}$
\Statex \textbf{Output:} Updated latents $\mathbf{z}_t$
\State $\mathbf{z}_t \gets \mathbf{z}_t.\operatorname{detach}().\operatorname{requires\_grad\_}(True)$
\For{each latent $\mathbf{z}_t^{(n)}$ and text embedding $\mathbf{E}^{(n)}$}
    \State Reset gradients
    \State Compute noise prediction and attention maps: \par
    \hskip\algorithmicindent $(\boldsymbol{\epsilon}_\theta, \mathbf{A}_t) \gets \text{SD}(\mathbf{z}_t^{(n)}, P, t, \mathbf{E}^{(n)})$
    \State Aggregate attention maps: \par
    \hskip\algorithmicindent $\{\mathbf{A}_i\} \gets \operatorname{AggregateAttentionMaps}(\mathbf{A}_t)$
    \State Compute total loss: \par
    \hskip\algorithmicindent $\mathcal{L} = \lambda_{\text{div}} \mathcal{L}_{\text{div}} + \lambda_{\text{sim}} \mathcal{L}_{\text{sim}} + \lambda_{\text{out}} \mathcal{L}_{\text{out}} + \lambda_{\text{PAC}} \mathcal{R}_{\text{PAC}}$
    \If{$i < K$}
        \State Update latent: $\mathbf{z}_t^{(n)} \gets \mathbf{z}_t^{(n)} - \alpha_t \nabla_{\mathbf{z}_t^{(n)}} \mathcal{L}$
    \EndIf
\EndFor
\State \textbf{Return} $\mathbf{z}_t$
\end{algorithmic}
\end{algorithm}


\section{Experiment}

\begin{table}[h!]
    \centering
    \begin{tabular}{|c|c c|}
        \hline
        \textbf{Model} & \textbf{Score} & \textbf{Change (\%)} \\
        \hline
        Ours & 0.344 & -- \\
        \hline
        - $R_{PAC}$ & 0.338 & \textcolor{red!70!black}{-1.74\%} \\
        \hline
        - $L_{out}$ & 0.336 & \textcolor{red!70!black}{-0.59\%} \\
        \hline
        - $L_{sim}$ & 0.331 & \textcolor{red!70!black}{-1.48\%} \\
        \hline
    \end{tabular}
    \caption{ABC-6K Dataset}
\end{table}

We evaluate our method on benchmark datasets, including the Attend-and-Excite dataset~\cite{Chefer23}, the ABC-6K dataset, and the DVMP dataset~\cite{Rassin23}, to assess its effectiveness in enhancing attribute binding and object representation in text-to-image generation. Comparisons are made with state-of-the-art models such as Stable Diffusion~\cite{Rombach22}, Attend-and-Excite~\cite{Chefer23}, and EBAMA~\cite{Zhang24}. Quantitative evaluations utilize CLIP similarity scores~\cite{Radford21}, measuring the alignment between generated images and textual prompts. Our method achieves higher CLIP scores across various prompt types, indicating improved attribute-object alignment and reduced object neglect. For instance, on the Attend-and-Excite dataset, our approach outperforms baselines in both full and minimum similarity metrics. Qualitative analyses also demonstrate that our model generates images with correct attribute associations and includes all specified elements from the prompts. An ablation study confirms that each component of our loss function contributes to performance gains, validating the effectiveness of our Bayesian framework in guiding attention mechanisms.



\section{Conclusion}

Our proposed method effectively guides the attention mechanism in text-to-image diffusion models, particularly when processing prompts with multiple objects. By addressing the challenges of balanced attention allocation, correct attribute association, and generalization, our approach enhances the quality and coherence of the generated images. The integration of the PAC-Bayes regularizer further strengthens the model's robustness by preventing overfitting to specific attention patterns.


%------------------------------------------------------------------------

==> sec/0_pre_1.tex <==
%3. 4.3.1 往前放，我们希望attation map 有哪些特点。 试了很多不同的prior，选了4个。 User should design their own prior，只不过我们做了这样的，其他人也可以这样做，突出bayesion framework novelity

%5. Method 先讲problem formulation。不要加一些新的notation。 Problem: prompt -> token (4.2.1)
%6. Better loss name for outside loss.

\section{Introduction} \label{sec
}

Text-to-image diffusion models have revolutionized the field of generative modeling, enabling the creation of high-fidelity images conditioned on textual descriptions~\cite{Rombach22,Nichol21,Saharia22,Ho20,Dhariwal21,Song21,Kingma21}. These models have demonstrated remarkable capabilities in generating diverse and realistic images, pushing the boundaries of creativity and visual representation~\cite{Radford21,Esser21,Dosovitskiy21,Brock19,Goodfellow14,Reed2016generative}. Techniques like classifier-free guidance~\cite{Ho2022classifier} and improved training strategies~\cite{Nichol2021improved} have further enhanced their performance. Despite their impressive achievements, these models often face challenges when handling complex prompts containing multiple objects and attributes~\cite{Zhang24,Chefer23,Feng23,Liu22,Rassin23}. Specifically, they may struggle with correctly associating modifiers to the appropriate nouns and allocating balanced attention among different elements in the prompt, leading to images that do not accurately reflect the intended description~\cite{Rassin23,Chefer23,Zhang24, chang2024skews, zhang2024objectconditioned}.

The problem of attribute misbinding and object neglect in text-to-image generation has been extensively studied~\cite{Zhang24,Rassin23,Chefer23,Zhang2023adding,Park23,Agarwal23}. For instance, Zhang et al.\cite{Zhang24} observed that diffusion models may generate images with incorrect attribute bindings or completely neglect certain objects mentioned in the prompt. Similarly, Chefer et al.\cite{Chefer23} introduced the \emph{Attend-and-Excite} method to enhance object presence but noted that it may lead to attribute leakage and artifacts. Rassin et al.\cite{Rassin23} highlighted the limitations of existing attention mechanisms in correctly capturing attribute-object relationships. Moreover, issues such as object hallucination\cite{Kim2022diffusionclip}, semantic confusion~\cite{Gal2022an}, and context misalignment~\cite{Li2023gligen} further exacerbate these challenges.

A significant part of this challenge stems from the attention mechanisms within these models, which often function as black boxes~\cite{Esser21,Rassin23,Feng23,Hertz23,Vaswani17}. The lack of transparency and control over attention distributions makes it difficult to guide the model towards desired behaviors, such as correct attribute binding and balanced attention allocation~\cite{Hertz23,Avrahami2022blended,Brooks2023instructpix2pix}. Without a way to influence the attention maps, users have limited ability to correct misalignments between the textual input and the generated images~\cite{Hertz23,Chefer23,Rassin23}.

Several approaches have been proposed to address these issues. Hertz et al.\cite{Hertz23} introduced \emph{Prompt-to-Prompt} editing, allowing users to control the generation process by manipulating cross-attention maps. Liu et al.\cite{Liu22} proposed \emph{Composable Diffusion} models that compose multiple outputs guided by different objects in the text prompt. Feng et al.\cite{Feng23} presented \emph{Training-Free Structured Diffusion Guidance} to enhance compositionality in text-to-image synthesis. However, these methods may still suffer from attribute misbinding and lack theoretical guarantees on their generalization performance\cite{Zhang24,Chefer23}.

Recently, Zhang et al.\cite{Zhang24} introduced an \emph{Object-Conditioned Energy-Based Attention Map Alignment} (EBAMA) method to address attribute binding and object neglect problems. Their approach leverages an energy-based model to align attention maps between attributes and objects, improving semantic alignment. While effective, their method focuses on specific energy functions and may not provide a flexible framework for designing custom attention priors\cite{Park23}. Additionally, methods like \emph{A-STAR}\cite{Agarwal23} and \emph{GLIGEN}\cite{Li2023gligen} have attempted to incorporate external knowledge or grounding mechanisms but may introduce additional complexity.

In this paper, we propose a novel Bayesian framework to guide the attention mechanisms in text-to-image diffusion models. By formalizing the problem within the PAC-Bayes framework~\cite{McAllester99}, we provide a principled approach that allows users to design their own priors over attention distributions, specifying desirable characteristics for the attention maps. We experimented with various priors and selected key components that enforce attention map properties such as divergence between different objects, similarity between modifiers and their corresponding nouns, minimal attention to irrelevant tokens, and regularization to prevent overfitting.

Our approach differs from previous works in that it treats the attention mechanism not as a black box, but as an interpretable component that can be guided using Bayesian principles. By minimizing the Kullback-Leibler divergence between the learned attention distributions and the designed priors, we effectively guide the model to produce images with better attribute-object alignment and balanced attention allocation. Importantly, this framework is flexible, allowing users to define their own priors based on specific needs or preferences, thereby highlighting the novelty and versatility of our Bayesian approach.

Our contributions can be summarized as follows:

\begin{itemize} \item We introduce a novel Bayesian framework that allows for the design of custom priors over attention distributions in text-to-image diffusion models, enhancing control over the attention mechanism and addressing the black-box nature of existing models. \item We formalize the problem within the PAC-Bayes framework~\cite{McAllester99}, providing theoretical guarantees on the generalization performance and highlighting the novelty of our approach. \item We demonstrate that our method achieves state-of-the-art results on standard benchmarks~\cite{Chefer23, Feng23, Rassin23}, improving attribute binding accuracy and attention allocation in generated images, thus validating the effectiveness of our framework. \end{itemize}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.51\textwidth]{photo/flow_1.png} %0.475
    \caption{\textbf{An overview of our workflow for optimizing the stable diffusion model.} It includes aggregation of attention maps, computation of object-centric attention loss, and updates to $z_t$.}
    \label{fig:flow_image}
\end{figure}

\section{Related Works}

\subsection{Stable Diffusion}

Stable Diffusion~\cite{Rombach22} is a seminal work in text-to-image synthesis that employs a latent diffusion model to generate high-resolution images efficiently. By operating in a lower-dimensional latent space \cite{yu2024latent} learned through an autoencoder~\cite{Esser21,Rombach21}, Stable Diffusion significantly reduces computational requirements compared to pixel-space diffusion models~\cite{Sohl-Dickstein2015deep,Ho20,Dhariwal21}. It leverages cross-attention mechanisms~\cite{Vaswani17,Parmar2018image} to align textual and visual information, enabling the generation of diverse and detailed images conditioned on textual prompts~\cite{Nichol21,Saharia22, Li2023}. Techniques such as classifier-free guidance~\cite{Ho2022classifier} and improved training objectives~\cite{Nichol2021improved} have further enhanced the quality and controllability of generated images \cite{zhang2024flow, zhu2024think}. However, despite its success, Stable Diffusion and similar models often struggle with complex prompts involving multiple objects and attributes~\cite{Rassin23,Chefer23,Feng23}, leading to issues such as attribute misbinding and object neglect.

\subsection{Bayesian Learning and PAC-Bayes Framework}

The PAC-Bayes framework~\cite{McAllester99} provides theoretical tools for analyzing the generalization performance of learning algorithms, especially those involving stochastic predictors \cite{zhang2024statistical}. By incorporating prior knowledge in the form of a prior distribution over hypotheses, PAC-Bayes offers generalization bounds that can guide model selection and regularization. Bayesian methods have been applied to various domains in machine learning, including neural networks and attention mechanisms~\cite{Ho2022classifier,Meng2021sdedit}, offering a principled way to incorporate uncertainty and prior information. In the context of diffusion models, Bayesian approaches have been used to improve image restoration~\cite{Kawar2022denoising} and editing~\cite{Avrahami2022blended}. In our work, we adopt the PAC-Bayes framework to design custom priors over attention distributions in diffusion models, enabling controlled and interpretable attention mechanisms that improve attribute-object alignment.

%-------------------------------------------------------------------------


\section{Background}
\label{sec:background}

\subsection{Stable Diffusion Models}

Stable Diffusion Models (SD)~\cite{Rombach22}. SD first encodes an image \( x \) into the latent space using a pretrained encoder~\cite{Esser21}, i.e., \( z = E(x) \). Given a text prompt \( y \), SD optimizes the conditional denoising autoencoder \( \epsilon_\theta \) by minimizing the objective:

\begin{equation}
\mathcal{L}_\theta = \mathbb{E}_{t, \epsilon \sim \mathcal{N}(0,1), z \sim \mathcal{E}(x)} \left\| \epsilon - \epsilon_\theta(z_t, t, \phi(y)) \right\|^2,
\label{eq:sd_loss}
\end{equation}

where \( \phi \) is a frozen CLIP text encoder~\cite{Radford21}, \( z_t \) is a noised version of the latent \( z \), and the time step \( t \) is uniformly sampled from \( \{1, \dots, T\} \). During sampling, \( z_T \) is randomly sampled from standard Gaussian and denoised iteratively by the denoising autoencoder \( \epsilon_\theta \) from time \( T \) to \( 0 \). Finally, a decoder \( D \) reconstructs the image as \( \tilde{x} = D(z_0) \).

\subsection{Cross-Attention Mechanism}

In the cross-attention mechanism, \( K \) is the linear projection of \( W_y \), the CLIP-encoded text embeddings of text prompt \( y \). \( Q \) is the linear projection of the intermediate image representation parameterized by latent variables \( z \). Given a set of queries \( Q \) and keys \( K \), the (unnormalized) attention features and (softmax-normalized) scores between these two matrices are:

\begin{equation}
A = \frac{Q K^\top}{\sqrt{m}}, \quad \tilde{A} = \text{softmax} \left( \frac{Q K^\top}{\sqrt{m}} \right),
\label{equ:attn}
\end{equation}

where \( m \) is the feature dimension. We consider both attention features and scores for our modeling here, which we denote as \( A_s \) and \( \tilde{A}_s \) for token \( s \), respectively.

%-------------------------------------------------------------------------
\begin{algorithm}[t]
\caption{A Single Denoising Step using PAC}
\label{alg:syngen_step}
\begin{algorithmic}[1]
\Statex \textbf{Input:} Text prompt $P$, latents $\mathbf{z}_t$, text embeddings $\mathbf{E}$, timestep $t$, iteration $i$, step size $\alpha_t$, number of intervention steps $K$, trained Stable Diffusion model $\text{SD}$, loss hyperparameters $\lambda_{\text{div}}$, $\lambda_{\text{sim}}$, $\lambda_{\text{out}}$, $\lambda_{\text{PAC}}$
\Statex \textbf{Output:} Updated latents $\mathbf{z}_t$
\State $\mathbf{z}_t \gets \mathbf{z}_t.\operatorname{detach}().\operatorname{requires\_grad\_}(True)$
\For{each latent $\mathbf{z}_t^{(n)}$ and text embedding $\mathbf{E}^{(n)}$}
    \State Reset gradients
    \State Compute noise prediction and attention maps: \par
    \hskip\algorithmicindent $(\boldsymbol{\epsilon}_\theta, \mathbf{A}_t) \gets \text{SD}(\mathbf{z}_t^{(n)}, P, t, \mathbf{E}^{(n)})$
    \State Aggregate attention maps: \par
    \hskip\algorithmicindent $\{\mathbf{A}_i\} \gets \operatorname{AggregateAttentionMaps}(\mathbf{A}_t)$
    \State Compute total loss: \par
    \hskip\algorithmicindent $\mathcal{L} = \lambda_{\text{div}} \mathcal{L}_{\text{div}} + \lambda_{\text{sim}} \mathcal{L}_{\text{sim}} + \lambda_{\text{out}} \mathcal{L}_{\text{out}} + \lambda_{\text{PAC}} \mathcal{R}_{\text{PAC}}$
    \If{$i < K$}
        \State Update latent: $\mathbf{z}_t^{(n)} \gets \mathbf{z}_t^{(n)} - \alpha_t \nabla_{\mathbf{z}_t^{(n)}} \mathcal{L}$
    \EndIf
\EndFor
\State \textbf{Return} $\mathbf{z}_t$
\end{algorithmic}
\end{algorithm}

\section{Method and Theoretical Foundations}
\label{sec:method}

In this section, we introduce our method designed to guide the attention mechanism of text-to-image diffusion models when processing prompts containing multiple objects. Our approach leverages the attention maps produced by the model to ensure balanced attention, correct attribute association, and improved generalization.

\subsection{Attention Map Distribution}

We focus on the extraction of nouns and modifiers from the text prompt and how the model can find their interactions. For example, given a prompt like \emph{"a yellow bird and a blue lion"}, we use a natural language parser to identify the nouns (\emph{"bird"}, \emph{"lion"}) and modifiers (\emph{"yellow"}, \emph{"blue"}), and determine the associations between them.

By analyzing the syntactic structure of the prompt, the parser can identify that \emph{"yellow"} modifies \emph{"bird"}, and not \emph{"lion"}. This information is crucial for guiding the attention mechanism so that the model correctly associates attributes with the corresponding objects in the generated image.

Our method utilizes spaCy’s transformer-based dependency parser \cite{spacy2}, which can maps the tokens in the prompt to their corresponding attention maps. By aligning the attention maps with the syntactic structure of the prompt, we can enforce constraints that encourage the model to attend appropriately to different parts of the image during generation.

\subsection{PAC-Bayes Framework}

To formalize our approach, we employ the PAC-Bayes framework~\cite{McAllester99}, which provides a theoretical foundation for understanding the generalization properties of learning algorithms.

\begin{definition}[PAC-Bayes Bound]
Given a prior distribution \( P \) over hypotheses \( h \in \mathcal{H} \), with probability at least \( 1 - \delta \), the following inequality holds:

\begin{equation}
\begin{aligned}
\mathbb{E}_{h \sim Q} [\text{Risk}(h)] &\leq \mathbb{E}_{h \sim Q} [\widehat{\text{Risk}}(h)] + \\
&\quad \sqrt{ \frac{ D_{\text{KL}}(Q \parallel P) + \ln \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
\end{aligned}
\label{eq:pac_bayes_bound}
\end{equation}

where \( Q \) is the posterior distribution over hypotheses, \( \text{Risk}(h) \) is the true risk, \( \widehat{\text{Risk}}(h) \) is the empirical risk, \( D_{\text{KL}}(Q \parallel P) \) is the Kullback-Leibler divergence between \( Q \) and \( P \), \( N \) is the number of samples, and \( \delta \) is the confidence parameter (\( 0 < \delta < 1 \)).
\end{definition}

%\subsubsection{Why PAC-Bayes?}
The PAC-Bayes framework allows us to derive generalization bounds that depend on the divergence between the learned model and a prior belief. By incorporating prior knowledge about how attention should be distributed in the model (e.g., modifiers should be associated with their corresponding nouns), we can guide the learning process in a principled way.

Minimizing the KL divergence \( D_{\text{KL}}(Q \parallel P) \) ensures that the learned attention distributions \( Q \) are close to the prior \( P \), which encodes our desired properties. This helps to prevent overfitting and improves the generalization performance of the model.

\subsubsection{Representation of Attention Maps}

% We model the attention maps 
% as probability distributions 
% over a finite set \( \Omega \) (e.g., spatial locations in the image). Specifically, we represent each attention map \( A_i \) as a flattened vector of dimension \( n \times 1 \), where \( n \) is the number of elements (e.g., \( 16 \times 16 = 256 \) for a \( 16 \times 16 \) attention map). Each element \( A_i(j) \) satisfies:
% \begin{equation}
% A_i(j) \geq 0 \forall j \in \Omega; \quad \sum_{j \in \Omega} A_i(j) = 1,
% \label{eq:attention_distribution}
% \end{equation} 

We model the attention maps 
as probability distributions
over a finite set \( \Omega \). For attention map $A_i$,  we let \( \Omega_i \) denotes the spatial indices within the image. 
 Each entry \( A_i(j) \) represents a non-negative weight at spatial location $j$, satisfies:
\begin{equation}
A_i(j) \geq 0 \quad \forall j \in \Omega_i; \quad \sum_{j \in \Omega_i} A_i(j) = 1,
\label{eq:attention_distribution}
\end{equation} 

This ensures that the attention maps are valid probability distributions (i.e., multinomial distributions), facilitating the use of information-theoretic measures like the KL divergence.

% We represent each attention map \( A_i \) as a flattened vector of dimension \( n \times 1 \), where \( n \) is the number of elements (e.g., \( 16 \times 16 = 256 \) for a \( 16 \times 16 \) attention map). 

\begin{figure*}[th]
    \centering
    \includegraphics[width= \textwidth]{photo/photo_4.png}
    \caption{\textbf{Qualitative comparison on the AnE dataset (the left two columns) and the DVMP dataset (the right two columns).} We compared our model using the same prompt and random seed as SD \cite{Rombach21}, SG \cite{Rassin23}, AnE \cite{Chefer23}, and EMAMA \cite{Zhang24}, with each column sharing the same random seed.}

    \label{fig:body_image}
\end{figure*}

\begin{figure*}[th]
    \centering
    \includegraphics[width=\textwidth]{photo/photo_3.png}
    \caption{\textbf{Qualitative comparison on the ABC-6K dataset.} We compared our model using the same prompt and random seed as SD \cite{Rombach21}, SG \cite{Rassin23}, AnE \cite{Chefer23}, and EMAMA \cite{Zhang24}, with each column sharing the same random seed.}
    \label{fig:body_image}
\end{figure*}





\subsection{Our Algorithm}

From the PAC-Bayes inequality in Equation~\eqref{eq:pac_bayes_bound}, we aim to minimize the KL divergence \( D_{\text{KL}}(Q \parallel P) \) between the posterior \( Q \) and the prior \( P \), while keeping \( N \) and \( \delta \) constant.

\subsubsection{Prior and Posterior Distributions}


Let the $U$ be the uniform distribution. The prior \( U \) is designed to capture our prior beliefs about the attention distributions.


We define the  distribution \( A \) over attention maps that encode our desired properties.

Specifically, we factorize \( A \) as:


{ \footnotesize
\begin{equation}
\begin{aligned} &A(l) \propto \\ \nonumber
&\frac{1}{Z} \prod_{i \in \mathcal{A}_1} \left( A_i(l) \right)^{\alpha \mathbf{1}_{\Omega_i}(l)} \prod_{j \in \mathcal{A}_2} \left( A_j(l) \right)^{\beta \mathbf{1}_{\Omega_j}(l)} \prod_{k \in \mathcal{A}_3} \left( A_k(l) \right)^{\gamma \mathbf{1}_{\Omega_k}(l)}, \label{eq:prior_factorization} \end{aligned}\end{equation}} where $Z$ is the normalization constant, where:
\begin{itemize}
    \item \( \mathcal A_1 \) corresponds to the divergence component, encouraging the attention maps of different objects to be separated.
    \item \( \mathcal A_2 \) corresponds to the similarity component, encouraging modifiers and their associated nouns to have similar attention maps.
    \item \( \mathcal A_3 \) corresponds to the outside component, discouraging attention to irrelevant tokens (e.g., articles like \emph{`a''}, \emph{the''}).
    % \item \( A_4 \) corresponds to the regularizer, promoting generalization and preventing overfitting.
\end{itemize}

The exponents \( \alpha, \beta, \gamma\) are nonnegative hyperparameters controlling the influence of each component, satisfying \( \alpha + \beta + \gamma = 1 \).

The prior \( U \) is designed to capture our prior beliefs about the attention distributions. 

% The likelihood \( P(B | A) \) models the probability of observing the data \( B \) (e.g., the latent variables \( z_t \)) given the attention maps \( A \). 

The posterior \( A \) represents the learned attention distributions given the data.

\subsubsection{KL Divergence}

PAC-Bayes theory relies on the KL divergence between the posterior and the prior: 

We have 
{ \footnotesize
\begin{align}
&D_{\text{KL}}(A \parallel U) = \sum_{l} A(l) \log \left( \frac{A(l)}{U(l)} \right) \nonumber 
% &= \sum_{l \in \Omega} A(l) \log \left( \frac{\frac{1}{Z} \prod_{i \in \mathcal{A}_1} \left( A_i(l) \right)^{\alpha \mathbf{1}_{\Omega_i}(l)} \prod_{j \in \mathcal{A}_2} \left( A_j(l) \right)^{\beta \mathbf{1}_{\Omega_j}(l)} \prod_{k \in \mathcal{A}_3} \left( A_k(l) \right)^{\gamma \mathbf{1}_{\Omega_k}(l)}}{U(l)} \right) \nonumber \\
\end{align}
}
Substituting the factorized \( A \) from Equation~\eqref{eq:prior_factorization}, we have:

{ \footnotesize
\begin{equation}
\begin{aligned}
\label{kl_derivation}
&D_{\text{KL}}(A \parallel U)
= \alpha \sum_{i \in \mathcal{A}_1} \sum_{l \in \Omega_i} A(l) \log \frac{A_i(l)}{U_i(l)} + \beta \sum_{j \in \mathcal{A}_2} \sum_{l \in \Omega_j} A(l) \log \frac{A_j(l)}{U_j(l)} \nonumber \\
&\quad + \gamma \sum_{k \in \mathcal{A}_3} \sum_{l \in \Omega_k} A(l) \log \frac{A_k(l)}{U_k(l)} - \log Z - C. \\
& =\alpha \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U) + \beta \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U)  + \gamma \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U)  \nonumber \\ &- \log Z - C,
\end{aligned}
\end{equation}
}
where $C$ is a constant. 

% Our goal is to minimize the KL divergence between the posterior and the prior:

% \begin{equation}
% D_{\text{KL}}(Q \parallel P) = \sum_{A} Q(A) \log \left( \frac{Q(A)}{P(A)} \right).
% \label{eq:kl_divergence_qp}
% \end{equation}

% Substituting the factorized prior \( P(A) \) from Equation~\eqref{eq:prior_factorization}, we have:



% { \footnotesize
% \begin{align}
% D_{\text{KL}}(Q \parallel P) &= \sum_{A} Q(A) \log \left( \frac{Q(A)}{\frac{1}{Z} \left( P_1(A) \right)^\alpha \left( P_2(A) \right)^\beta \left( P_3(A) \right)^\gamma \left( P_4(A) \right)^\eta} \right) \nonumber \\
% &= \sum_{A} Q(A) \log Q(A) \nonumber \\
% &\quad - \sum_{A} Q(A) \left( \alpha \log P_1(A) + \beta \log P_2(A) \right. \nonumber \\
% &\qquad \left. + \gamma \log P_3(A) + \eta \log P_4(A) - \log Z \right),
% \end{align}
% }

% { \footnotesize
% \begin{align*}
% D_{\text{KL}}(Q \parallel P) &= \sum_{A} Q(A) \log Q(A) - \alpha \sum_{A} Q(A) \log P_1(A) \\
% &\quad - \beta \sum_{A} Q(A) \log P_2(A) \\
% &\quad - \gamma \sum_{A} Q(A) \log P_3(A) - \eta \sum_{A} Q(A) \log P_4(A) + \text{Constant}.
% \end{align*}
% }

% where \( Z \) is the normalization constant. Since \( \log Z \) is a constant, we can omit it during optimization, resulting in: 

% % The KL divergence then becomes:




% % This can be rewritten as:
% { \footnotesize
% \begin{equation}
% \begin{aligned}
% D_{\text{KL}}(Q \parallel P) &= \alpha \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_1(A)} \right) + \beta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_2(A)} \right) \\
% &\quad + \gamma \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_3(A)} \right) + \eta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_4(A)} \right) \\
% &\quad + \left( 1 - \alpha - \beta - \gamma - \eta \right) \sum_{A} Q(A) \log Q(A) + \text{const}.
% \end{aligned}
% \end{equation}
% }
% { \footnotesize
% \begin{align}
% D_{\text{KL}}(Q \parallel P) &= \alpha \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_1(A)} \right) + \beta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_2(A)} \right) \nonumber \\
% &\quad + \gamma \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_3(A)} \right) + \eta \sum_{A} Q(A) \log \left( \frac{Q(A)}{P_4(A)} \right)\\
% & + \left( 1 - \alpha - \beta - \gamma - \eta \right) \sum_{A} Q(A) \log Q(A) + \text{const}.
% \end{align}
% }





Therefore, optimizing \( D_{\text{KL}}(A \parallel U) \) is equivalent to optimizing the weighted sum of KL divergences:

{ \footnotesize
\begin{align}
\label{kl_decomp}
D_{\text{KL}}(A \parallel U) &= \alpha \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U) + \beta \sum_{j \in \mathcal{A}_2} D_{\text{KL}}(A_j \parallel U) \nonumber \\
&\quad +   \gamma \sum_{k \in \mathcal{A}_3}D_{\text{KL}}(A_k \parallel U)  + \text{const}.
\end{align}
}









% \begin{equation}
%     \begin{aligned}
%      & D_{\text{KL}}(A \parallel U)   = \sum_{l\in \Omega} A(l) \log \Bigl(\frac{A(l)}{U(l)} \Bigr) \\
%       &= \sum_{l\in \Omega} A(l) \log \Bigl(\frac{\prod_{i\in \mathcal A_1}\left( A_i(l) \right)^\alpha \prod_{j\in \mathcal A_2} \left( A_j(l) \right)^\beta \prod_{j\in \mathcal A_2} \left( A_k(l) \right)^\gamma}{ZU(l)} \Bigr) \\
%       &=\sum A \alpha \sum_{i\in \mathcal A_1} \log(A_i) + \sum A \beta \sum_{j\in \mathcal A_2} \log(A_j) + \sum A \gamma \sum_{k\in \mathcal A_3} \log(A_k) \\ &- \sum A(\alpha |\mathcal A_1| + \beta |\mathcal A_2| + \gamma |\mathcal A_3|)|\Omega|
%     \end{aligned}
% \end{equation}
% { \footnotesize
% \begin{align}
% &D_{\text{KL}}(A \parallel U) = \sum_{l \in \Omega} A(l) \log \left( \frac{A(l)}{U(l)} \right) \nonumber \\
% &= \sum_{l \in \Omega} A(l) \log \left( \frac{\frac{1}{Z} \prod_{i \in \mathcal{A}_1} \left( A_i(l) \right)^{\alpha \mathbf{1}_{\Omega_i}(l)} \prod_{j \in \mathcal{A}_2} \left( A_j(l) \right)^{\beta \mathbf{1}_{\Omega_j}(l)} \prod_{k \in \mathcal{A}_3} \left( A_k(l) \right)^{\gamma \mathbf{1}_{\Omega_k}(l)}}{U(l)} \right) \nonumber \\
% &= \sum_{l \in \Omega} A(l) \left( \sum_{i \in \mathcal{A}_1} \alpha \mathbf{1}_{\Omega_i}(l) \log \frac{A_i(l)}{U_i(l)} + \sum_{j \in \mathcal{A}_2} \beta \mathbf{1}_{\Omega_j}(l) \log \frac{A_j(l)}{U_j(l)} + \sum_{k \in \mathcal{A}_3} \gamma \mathbf{1}_{\Omega_k}(l) \log \frac{A_k(l)}{U_k(l)} - \log Z - C \right) \nonumber \\
% &= \sum_{i \in \mathcal{A}_1} \alpha \sum_{l \in \Omega_i} A(l) \log \frac{A_i(l)}{U_i(l)} + \sum_{j \in \mathcal{A}_2} \beta \sum_{l \in \Omega_j} A(l) \log \frac{A_j(l)}{U_j(l)} + \sum_{k \in \mathcal{A}_3} \gamma \sum_{l \in \Omega_k} A(l) \log \frac{A_k(l)}{U_k(l)} \nonumber \\
% &\quad - \sum_{l \in \Omega} A(l) \log Z - C \nonumber \\
% &= \alpha \sum_{i \in \mathcal{A}_1} \sum_{l \in \Omega_i} A(l) \log \frac{A_i(l)}{U_i(l)} + \beta \sum_{j \in \mathcal{A}_2} \sum_{l \in \Omega_j} A(l) \log \frac{A_j(l)}{U_j(l)} \nonumber \\
% &\quad + \gamma \sum_{k \in \mathcal{A}_3} \sum_{l \in \Omega_k} A(l) \log \frac{A_k(l)}{U_k(l)} - \log Z - C. \\
% & =\alpha \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U) + \beta \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U)  + \gamma \sum_{i \in \mathcal{A}_1} D_{\text{KL}}(A_i \parallel U) 
% \end{align}
% }


\subsection{Final Loss Function}
Inspired by the derivation of KL divergence, it brings us to our total loss function, which combines the four components: divergence, similarity, outside, and regularization losses.

The final loss function we optimize is:

\begin{equation}
\mathcal{L}_{\text{total}} = \lambda_{\text{div}} \mathcal{L}_{\text{div}} + \lambda_{\text{sim}} \mathcal{L}_{\text{sim}} + \lambda_{\text{out}} \mathcal{L}_{\text{out}} + \lambda_{\text{PAC}} \mathcal{R}_{\text{PAC}},
\label{eq:total_loss_final}
\end{equation}

where \( \lambda_{\text{div}} = \alpha \), \( \lambda_{\text{sim}} = \beta \), \( \lambda_{\text{out}} = \gamma \), and \( \lambda_{\text{PAC}} = \eta \), corresponding to the exponents in the prior distribution.

By minimizing this loss according to the PAC-Bayes bound \cite{McAllester99}, we could control the generalization error of our model.

%In our setup, we consider a text prompt containing a total of \( n \) objects. We denote \( \mathcal{O} = \{1, 2, \dots, n\} \) as the set of object indices in the prompt, and for each object \( k \in \mathcal{O} \), we define the aggregated attention map \( A_{\text{obj}_k} \) by combining the attention maps of its noun and associated modifiers. This aggregated attention map represents the overall attention allocated to object \( k \) across different spatial locations in the generated image. Additionally, for each object \( k \), we have the sets \( \mathcal{M}_k \) and \( \mathcal{N}_k \), which are the sets of modifier (attribute) token indices and noun token indices associated with object \( k \), respectively. Given that modifiers may include adjectives or other descriptive words, while nouns represent the core object terms, we define \( \mathcal{S} \) as the set of all object-related token indices, given by \( \mathcal{S} = \bigcup_{k=1}^{n} (\mathcal{M}_k \cup \mathcal{N}_k) \). The set of outside (irrelevant) token indices is denoted by \( \mathcal{O}_{\text{outside}} \), which consists of all token indices in the prompt that are not in \( \mathcal{S} \). These may include articles, conjunctions, or other words that are not directly related to the objects. The attention map for each token \( i \) is denoted by \( A_i \), representing how much attention the model allocates to different spatial locations in the image when processing token \( i \). Each attention map \( A_i \) is a probability distribution over the set of spatial locations \( \Omega \), satisfying \( \sum_{l \in \Omega} A_i(l) = 1 \) and \( A_i(l) \geq 0 \) for all \( l \in \Omega \).

\subsubsection{Divergence Loss}

The divergence loss $\mathcal{L}_{\text{divergence}}$ measures the symmetric Kullback-Leibler (KL) divergence between the combined attention maps of the two objects in the prompt. This component encourages the model to allocate attention evenly between the objects.

%Let $A_{\text{object1}}$ and $A_{\text{object2}}$ denote the combined attention maps for object 1 and object 2, respectively. The divergence loss is defined as:

%Consider a text prompt with total $n$ number of objects, let \( \mathcal{O} = \{1, 2, \dots, n\} \) be the set of object indices in the prompt. For each object \( k \in \mathcal{O} \), we define the attention map \( A_{\text{obj}_k} \) by aggregating the attention maps of its noun and modifiers.


\begin{equation}
\mathcal{L}_{\text{divergence}} = - \frac{1}{2} \left[ D_{\text{KL}}(A_{\text{obj1}} \parallel A_{\text{obj2}}) + D_{\text{KL}}(A_{\text{obj2}} \parallel A_{\text{obj1}}) \right]
\label{eq:divergence_loss}
\end{equation} % 这个是个负值，不是正的。

For this loss, we want the two objects to be away from each other. By doing the KL convergence away from the object(1) attention map to object(2). The model can distinguish the difference between the two objects.  

\subsubsection{Similarity Loss}

The similarity loss $\mathcal{L}_{\text{similarity}}$ promotes coherence within each object by encouraging the attention maps of modifiers and nouns to be similar.

For each object $k \in \{1, 2\}$:

\begin{itemize}
    \item Let $\mathcal{M}_k$ be the set of modifier indices (e.g., adjectives).
    \item Let $\mathcal{N}_k$ be the set of noun indices.
    \item Define the set of modifier-noun pairs $\mathcal{P}_k = \{ (i, j) \mid i \in \mathcal{M}_k, \, j \in \mathcal{N}_k \}$.
\end{itemize}

The similarity loss for object $k$ is:

\begin{equation}
\mathcal{L}_{\text{similarity}}^{(k)} = \frac{1}{|\mathcal{P}_k|} \sum_{(i, j) \in \mathcal{P}_k} D_{\text{sym}}(A_i, A_j)
\label{eq:similarity_loss_k}
\end{equation}

where $D_{\text{sym}}(A_i, A_j)$ is the symmetric KL divergence between attention maps $A_i$ and $A_j$:

\begin{equation}
D_{\text{sym}}(A_i, A_j) = \frac{1}{2} \left[ D_{\text{KL}}(A_i \parallel A_j) + D_{\text{KL}}(A_j \parallel A_i) \right]
\label{eq:symmetric_kl}
\end{equation}

The total similarity loss is the sum over both objects:

\begin{equation}
\mathcal{L}_{\text{similarity}} = \mathcal{L}_{\text{similarity}}^{(1)} + \mathcal{L}_{\text{similarity}}^{(2)}
\label{eq:similarity_loss}
\end{equation}

Here this loss, we want to maximize the attention map of modifiers using KL correspond to their attention map of the object. For example, a pink crown and a purple bow, we want the attention map of pink and attention map of crown to be similar to each other. %这里比较像 Linguistic blinding 那篇论文。




\subsubsection{Outside Loss}

The outside loss $\mathcal{L}_{\text{outside}}$ discourages the attention maps of object tokens from being similar to those of unrelated tokens (outside tokens).

Let:

\begin{itemize}
    \item $\mathcal{S} = \mathcal{M}_1 \cup \mathcal{N}_1 \cup \mathcal{M}_2 \cup \mathcal{N}_2$: The set of all object token indices.
    \item $\mathcal{O} = \text{All Indices} \setminus \mathcal{S}$: The set of outside token indices.
\end{itemize}

The outside loss is defined as:

\begin{equation}
\mathcal{L}_{\text{outside}} = -\frac{1}{|\mathcal{S}|} \sum_{i \in \mathcal{S}} \left( \max_{j \in \mathcal{O}} D_{\text{sym}}(A_i, A_j) \right)
\label{eq:outside_loss}
\end{equation}

This loss component prevents the model from confusing object-specific tokens with unrelated tokens. By penalizing high similarity between them, the model learns to focus on relevant parts of the prompt, improving the clarity and accuracy of the generated images. % 这个写的没问题 像Snygen 那篇文章

\subsubsection{PAC-Bayes Regularizer}

The PAC-Bayes regularizer $\mathcal{R}_{\text{PAC}}$ incorporates principles from PAC-Bayes theory to regularize the attention distributions, promoting generalization.

Let $N$ be the number of samples and $\delta$ be the confidence parameter. The regularizer is computed as:

% \begin{equation}
% \mathcal{R}_{\text{PAC}} = -\sqrt{ \frac{ \left( \dfrac{1}{2} \sum\limits_{k=1}^{2} D_{\text{KL}}(A_{\text{object}k} \parallel U) \right) + \log \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
% \label{eq:pac_bayes_regularizer}
% \end{equation} % 应该是负数，应该离 uniform distribution 越远越好 


\begin{equation}
\mathcal{R}_{\text{PAC}} = -\sqrt{ \frac{   D_{\text{KL}}(A \parallel U)  + \log \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
\label{eq:pac_bayes_regularizer}
\end{equation} % 应该是负数，应该离 uniform distribution 越远越好 
Here, $U$ represents the uniform distribution over the attention map dimensions. 
% By \eqref{kl_decomp}, we have, 

% \begin{align}
%   &\mathcal{R}_{\text{PAC}}=\\ &  -\sqrt{ \frac{3\alpha\sum_{i\in\mathcal A_1}   D_{\text{KL}}(A_i \parallel U)  + \log \left( 2 \sqrt{N}/\delta \right) }{6N} }    
% \end{align}

The goal of this formula is to make the attention map away from the uniform distribution. The PAC prevents the model from becoming overly confident in specific attention patterns, prevents overfitting. 

(1) The PAC-Bayes feeds the not uniform distribution into the model as the prior 






\begin{table*}[t]
    \centering
    \label{tab:clip_scores}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|ccc|ccc|}
        \hline
        \textbf{Method} & \multicolumn{3}{c|}{\textbf{Animal-Animal}} & \multicolumn{3}{c|}{\textbf{Animal-Object}} & \multicolumn{3}{c|}{\textbf{Object-Object}} \\
        \hline
         & \textbf{Full Sim.} & \textbf{Min. Sim.} & \textbf{T-C Sim.} & \textbf{Full Sim.} & \textbf{Min. Sim.} & \textbf{T-C Sim.} & \textbf{Full Sim.} & \textbf{Min. Sim.} & \textbf{T-C Sim.} \\
        \hline
        SD \cite{Rombach22} & 0.311 & 0.213 & 0.767 & 0.340 & 0.246 & 0.793 & 0.335 & 0.235 & 0.765 \\
        CD \cite{Liu22} & 0.284 & 0.232 & 0.692 & 0.336 & 0.252 & 0.769 & 0.349 & 0.265 & 0.759 \\
        StrD \cite{Feng23} & 0.306 & 0.210 & 0.761 & 0.336 & 0.242 & 0.781 & 0.332 & 0.234 & 0.762 \\
        EBCA \cite{Park23} & 0.291 & 0.215 & 0.722 & 0.317 & 0.229 & 0.732 & 0.321 & 0.231 & 0.726 \\
        AnE \cite{Chefer23} & 0.332 & 0.248 & 0.806 & 0.353 & 0.265 & 0.830 & 0.360 & 0.270 & 0.811 \\
        SG \cite{Rassin23} & 0.311 & 0.213 & 0.767 & 0.355 & 0.264 & 0.830 & 0.355 & 0.262 & 0.811 \\
        EBAMA \cite{Zhang24} & 0.340 & 0.256 & 0.817 & 0.362 & 0.270 & 0.851 & 0.366 & 0.274 & 0.836 \\
        D\&B \cite{Li2023} & 0.331 & 0.246 & 0.810 & -- & -- & -- & -- & -- & -- \\
        \hline
        \textbf{Ours} & \textbf{0.348} & \textbf{0.262} & \textbf{0.823} & \textbf{0.370} & \textbf{0.276} & \textbf{0.868} & \textbf{0.370} & \textbf{0.275} & \textbf{0.844} \\
        \hline
    \end{tabular}
    }
    \caption{ \textbf{ Comparison of Full Sim., Min. Sim., and T-C Sim. across different methods on the AnE dataset. CLIP Score based on the Attend and Excite Dataset.} Note that the performance of SG on Animal-Animal is degraded to SD, as the prompts do not contain any attribute-object pairs. The best results for each category is marked in bold numbers.}

\end{table*}





\section{Workflow}

Our proposed method integrates custom attention priors into the denoising process of text-to-image diffusion models, specifically Stable Diffusion~\cite{Rombach22}. We begin by parsing the input prompt using a natural language parser to extract nouns and their associated modifiers, identifying the relationships between them. During each denoising step, we extract the cross-attention maps corresponding to these tokens. We then apply custom loss functions based on the Kullback-Leibler divergence between the learned attention distributions and our designed priors, guided by the PAC-Bayes framework~\cite{McAllester99}. This includes losses that encourage divergence between different objects' attention maps, similarity between modifiers and their nouns, minimal attention to irrelevant tokens, and a regularization term to prevent overfitting. By combining these losses, we update the latent representations iteratively, refining the generated image to better align with the input prompt and improving attribute binding accuracy.


Algorithm~\ref{alg:syngen_step} outlines a single denoising step using our proposed loss function.




\section{Experiment}

\begin{figure}[th]
    \centering
    \includegraphics[width=0.475\textwidth]{photo/photo_chart.png}
    \caption{ \textbf{Full Sim. results on DVMP and ABC-6K datasets.} We randomly sample 200 prompts from each dataset and generate 4 images for each prompt.}
    \label{fig:chart_image}
\end{figure}

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c c|}
        \hline
        \textbf{Model} & \textbf{Score} & \textbf{Change (\%)} \\
        \hline
        Ours & 0.344 & -- \\
        \hline
        - $R_{PAC}$ & 0.338 & \textcolor{red!70!black}{-1.74\%} \\
        \hline
        - $L_{out}$ & 0.336 & \textcolor{red!70!black}{-0.59\%} \\
        \hline
        - $L_{sim}$ & 0.331 & \textcolor{red!70!black}{-1.48\%} \\
        \hline
    \end{tabular}
    \caption{ABC-6K Dataset}
\end{table}

We evaluate our method on benchmark datasets, including the Attend-and-Excite dataset~\cite{Chefer23}, the ABC-6K dataset, and the DVMP dataset~\cite{Rassin23}, to assess its effectiveness in enhancing attribute binding and object representation in text-to-image generation. Comparisons are made with state-of-the-art models such as Stable Diffusion~\cite{Rombach22}, Attend-and-Excite~\cite{Chefer23}, and EBAMA~\cite{Zhang24}. Quantitative evaluations utilize CLIP similarity scores~\cite{Radford21}, measuring the alignment between generated images and textual prompts. Our method achieves higher CLIP scores across various prompt types, indicating improved attribute-object alignment and reduced object neglect. For instance, on the Attend-and-Excite dataset, our approach outperforms baselines in both full and minimum similarity metrics. Qualitative analyses also demonstrate that our model generates images with correct attribute associations and includes all specified elements from the prompts. An ablation study confirms that each component of our loss function contributes to performance gains, validating the effectiveness of our Bayesian framework in guiding attention mechanisms.

\begin{figure}[th]
    \centering
    \includegraphics[width=0.475\textwidth]{photo/photo_compare.png}
    \caption{ ... }
    \label{fig:comparison}
\end{figure}

\section{Conclusion}

Our proposed method effectively guides the attention mechanism in text-to-image diffusion models, particularly when processing prompts with multiple objects. By addressing the challenges of balanced attention allocation, correct attribute association, and generalization, our approach enhances the quality and coherence of the generated images. The integration of the PAC-Bayes regularizer further strengthens the model's robustness by preventing overfitting to specific attention patterns.


%------------------------------------------------------------------------

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}







\section{Method}
\label{sec:method}


\subsection{Total Loss Function}

The total loss function $\mathcal{L}_{\text{total}}$ combines all four components and is defined as:

\begin{equation}
\mathcal{L}_{\text{total}} = \lambda_{\text{div}} \cdot \mathcal{L}_{\text{div}} + \lambda_{\text{sim}} \cdot \mathcal{L}_{\text{sim}} + \lambda_{\text{out}} \cdot \mathcal{L}_{\text{out}} + \lambda_{\text{PAC}} \cdot \mathcal{R}_{\text{PAC}}
\label{eq:total_loss}
\end{equation}

Here, $\lambda_{\text{div}}$, $\lambda_{\text{sim}}$, $\lambda_{\text{out}}$, and $\lambda_{\text{PAC}}$ are hyperparameters that control the contribution of each loss component.


\subsection{Divergence Loss}

The divergence loss $\mathcal{L}_{\text{divergence}}$ measures the symmetric Kullback-Leibler (KL) divergence between the combined attention maps of the two objects in the prompt. This component encourages the model to allocate attention evenly between the objects.

Let $A_{\text{object1}}$ and $A_{\text{object2}}$ denote the combined attention maps for object 1 and object 2, respectively. The divergence loss is defined as:

\begin{equation}
\mathcal{L}_{\text{divergence}} = - \frac{1}{2} \left[ D_{\text{KL}}(A_{\text{obj1}} \parallel A_{\text{obj2}}) + D_{\text{KL}}(A_{\text{obj2}} \parallel A_{\text{obj1}}) \right]
\label{eq:divergence_loss}
\end{equation} % 这个是个负值，不是正的。

For this loss, we want the two objects to be away from each other. By doing the KL convergence away from the object(1) attention map to object(2). The model can distinguish the difference between the two objects.  % 这个是和 A-star 和AnE 那一篇论文比较像 (晚一点润色）



\subsection{Similarity Loss}

The similarity loss $\mathcal{L}_{\text{similarity}}$ promotes coherence within each object by encouraging the attention maps of modifiers and nouns to be similar.

For each object $k \in \{1, 2\}$:

\begin{itemize}
    \item Let $\mathcal{M}_k$ be the set of modifier indices (e.g., adjectives).
    \item Let $\mathcal{N}_k$ be the set of noun indices.
    \item Define the set of modifier-noun pairs $\mathcal{P}_k = \{ (i, j) \mid i \in \mathcal{M}_k, \, j \in \mathcal{N}_k \}$.
\end{itemize}

The similarity loss for object $k$ is:

\begin{equation}
\mathcal{L}_{\text{similarity}}^{(k)} = \frac{1}{|\mathcal{P}_k|} \sum_{(i, j) \in \mathcal{P}_k} D_{\text{sym}}(A_i, A_j)
\label{eq:similarity_loss_k}
\end{equation}

where $D_{\text{sym}}(A_i, A_j)$ is the symmetric KL divergence between attention maps $A_i$ and $A_j$:

\begin{equation}
D_{\text{sym}}(A_i, A_j) = \frac{1}{2} \left[ D_{\text{KL}}(A_i \parallel A_j) + D_{\text{KL}}(A_j \parallel A_i) \right]
\label{eq:symmetric_kl}
\end{equation}

The total similarity loss is the sum over both objects:

\begin{equation}
\mathcal{L}_{\text{similarity}} = \mathcal{L}_{\text{similarity}}^{(1)} + \mathcal{L}_{\text{similarity}}^{(2)}
\label{eq:similarity_loss}
\end{equation}

Here this loss, we want to maximize the attention map of modifiers using KL correspond to their attention map of the object. For example, a pink crown and a purple bow, we want the attention map of pink and attention map of crown to be similar to each other. %这里比较像 Linguistic blinding 那篇论文。



\subsection{Outside Loss}

The outside loss $\mathcal{L}_{\text{outside}}$ discourages the attention maps of object tokens from being similar to those of unrelated tokens (outside tokens).

Let:

\begin{itemize}
    \item $\mathcal{S} = \mathcal{M}_1 \cup \mathcal{N}_1 \cup \mathcal{M}_2 \cup \mathcal{N}_2$: The set of all object token indices.
    \item $\mathcal{O} = \text{All Indices} \setminus \mathcal{S}$: The set of outside token indices.
\end{itemize}

The outside loss is defined as:

\begin{equation}
\mathcal{L}_{\text{outside}} = -\frac{1}{|\mathcal{S}|} \sum_{i \in \mathcal{S}} \left( \max_{j \in \mathcal{O}} D_{\text{sym}}(A_i, A_j) \right)
\label{eq:outside_loss}
\end{equation}

This loss component prevents the model from confusing object-specific tokens with unrelated tokens. By penalizing high similarity between them, the model learns to focus on relevant parts of the prompt, improving the clarity and accuracy of the generated images. % 这个写的没问题 像Snygen 那篇文章

\subsection{PAC-Bayes Regularizer}

The PAC-Bayes regularizer $\mathcal{R}_{\text{PAC}}$ incorporates principles from PAC-Bayes theory to regularize the attention distributions, promoting generalization.

Let $N$ be the number of samples and $\delta$ be the confidence parameter. The regularizer is computed as:

\begin{equation}
\mathcal{R}_{\text{PAC}} = -\sqrt{ \frac{ \left( \dfrac{1}{2} \sum\limits_{k=1}^{2} D_{\text{KL}}(A_{\text{object}k} \parallel U) \right) + \log \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
\label{eq:pac_bayes_regularizer}
\end{equation} % 应该是负数，应该离 uniform distribution 越远越好 

Here, $U$ represents the uniform distribution over the attention map dimensions.

The goal of this formula is to make the attention map away from the uniform distribution. The PAC prevents the model from becoming overly confident in specific attention patterns, prevents overfitting. 

(1) The PAC-Bayes feeds the not uniform distribution into the model as the prior 


\section{Theoretical Foundations}
\label{sec:theory}

In this section, we provide the theoretical underpinnings of our proposed loss function for guiding the attention mechanism in text-to-image diffusion models when processing prompts with two objects. We establish assumptions about the attention distributions, define necessary preliminaries, and present lemmas and theorems that justify the design of our loss components.

\subsection{Assumptions}

\textbf{Assumption 1 (Valid Attention Distributions).}
The attention maps \( A_i \) are valid probability distributions over a finite set \( \Omega \) (e.g., spatial locations or feature channels). Specifically, for each attention map \( A_i \):

\begin{equation}
A_i(j) \geq 0, \quad \forall j \in \Omega; \quad \sum_{j \in \Omega} A_i(j) = 1.
\label{eq:attention_distribution}
\end{equation}

This ensures that information-theoretic measures like the KL divergence are well-defined.

\textbf{Assumption 2 (Uniform Prior Distribution).}
For the PAC-Bayes regularizer, the prior distribution over attention maps is the uniform distribution \( U \), where:

\begin{equation}
U(j) = \dfrac{1}{|\Omega|}, \quad \forall j \in \Omega.
\label{eq:uniform_prior}
\end{equation}

This reflects a state of maximum uncertainty before observing any data.

\textbf{Assumption 3 (Finite Sample Size).}
We have a finite number \( N \) of samples (e.g., prompts), and the confidence parameter \( \delta \) satisfies \( 0 < \delta < 1 \).

\subsection{Preliminaries}

\textbf{Definition 1 (Kullback-Leibler Divergence).}
The Kullback-Leibler (KL) divergence between two probability distributions \( P \) and \( Q \) over the same finite set \( \Omega \) is defined as:

\begin{equation}
D_{\text{KL}}(P \parallel Q) = \sum_{j \in \Omega} P(j) \log \frac{P(j)}{Q(j)}.
\label{eq:kl_divergence}
\end{equation}

\textbf{Definition 2 (Symmetric KL Divergence).}
The symmetric KL divergence between two probability distributions \( P \) and \( Q \) is:

\begin{equation}
D_{\text{sym}}(P, Q) = \frac{1}{2} \left[ D_{\text{KL}}(P \parallel Q) + D_{\text{KL}}(Q \parallel P) \right].
\label{eq:symmetric_kl_divergence}
\end{equation}

\textbf{Definition 3 (PAC-Bayes Theorem).}
Given a prior distribution \( P \) and a posterior distribution \( Q \) over hypotheses $h\in \mathcal H$, where $\mathcal H$ is a function class, with probability at least \( 1 - \delta \), the following holds:

\begin{equation}
\begin{aligned}
\mathbb{E}_{h \sim Q} [\text{Risk}(h)] &\leq \mathbb{E}_{h \sim Q} [\widehat{\text{Risk}}(h)] + \\
&\quad \sqrt{ \frac{ D_{\text{KL}}(Q \parallel P) + \ln \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} }
\end{aligned}
\label{eq:pac_bayes_bound}
\end{equation}


where \( \text{Risk}(h) \) is the true risk (expected loss), and \( \widehat{\text{Risk}}(h) \) is the empirical risk (training loss).


\subsection{Key Lemmas}

\begin{lemma}[Non-negativity of KL Divergence]
\label{Lemma_1}
For any two attention distributions \( A_i \) and \( A_j \):

\begin{equation}
D_{\text{KL}}(A_i \parallel A_j) \geq 0.
\label{eq:kl_nonneg}
\end{equation}
    
\end{lemma}

\begin{proof}
This is a fundamental property of the KL divergence due to the Gibbs inequality.    
\end{proof}

\begin{lemma}[Properties of the Loss Components]
Each component of our loss function is non-negative:

\begin{equation}
\mathcal{L}_{\text{divergence}} \geq 0, \quad \mathcal{L}_{\text{similarity}} \geq 0, \quad \mathcal{L}_{\text{outside}} \geq 0.
\label{eq:loss_nonneg}
\end{equation}    
\end{lemma}
\begin{proof}
Since each loss component is defined using the symmetric KL divergence, which is non-negative (as per \cref{Lemma_1}), their sums and averages are also non-negative.    
\end{proof}


\subsection{Main Theorems}

\begin{theorem}[Effectiveness of Loss Components]
\label{theorem_1}
Minimizing each component of the loss function \( \mathcal{L}_{\text{total}} \) leads to specific desirable properties:

\begin{enumerate}
    \item \textbf{Divergence Loss (\( \mathcal{L}_{\text{divergence}} \))}: Promotes balanced attention between the two objects.
    \item \textbf{Similarity Loss (\( \mathcal{L}_{\text{similarity}} \))}: Ensures correct association between modifiers and nouns within each object.
    \item \textbf{Outside Loss (\( \mathcal{L}_{\text{outside}} \))}: Enhances distinction between object tokens and unrelated tokens.
    \item \textbf{PAC-Bayes Regularizer (\( \mathcal{R}_{\text{PAC}} \))}: Regularizes the attention distributions to prevent overfitting and improve generalization.
\end{enumerate}    
\end{theorem}
% \textbf{Theorem 1 (Effectiveness of Loss Components).}

\emph{Proof.}
Each loss component is designed to influence the attention distributions in a specific way.

%1. \textbf{Divergence Loss}: By minimizing the symmetric KL divergence between the combined attention maps of the two objects, we encourage the model to allocate attention more equally, preventing one object from dominating.

%2. \textbf{Similarity Loss}: Aligning the attention maps of modifiers and nouns ensures that attributes are correctly associated with their respective objects.

%3. \textbf{Outside Loss}: Penalizing high similarity between object tokens and outside tokens discourages the model from confusing relevant and irrelevant parts of the prompt.

%4. \textbf{PAC-Bayes Regularizer}: By penalizing the KL divergence from the uniform prior, we control the complexity of the attention distributions, reducing the risk of overfitting.
\textcolor{blue}{Todo: make clear about $A_{object k}$ in (7) and $Q$ in (15)}

\begin{theorem}[Generalization Bound via PAC-Bayes]
\label{theorem_2}
Under the PAC-Bayes framework and Assumptions 1 and 2, with probability at least \( 1 - \delta \), the expected loss over new samples is bounded by:

\begin{equation}
\begin{aligned}
\mathbb{E}_{A \sim Q} [\ell(A)] &\leq \frac{1}{N} \sum_{i=1}^N \ell(A_i) * \\
&\quad \sqrt{ \frac{ D_{\text{KL}}(Q \parallel U) + \ln \left( \dfrac{2 \sqrt{N}}{\delta} \right) }{2N} },
\end{aligned}
\label{eq:generalization_bound}
\end{equation}

where \( Q \) is the learned distribution over attention maps.   
\end{theorem}
% \textbf{Theorem 2 (Generalization Bound via PAC-Bayes).}
\emph{Proof.}
This is a direct application of the PAC-Bayes inequality (Equation \ref{eq:pac_bayes_bound}), where we consider the attention distributions as hypotheses and use the uniform prior \( U \).




\textbf{Gradient of Outside Loss}

The gradient of the outside loss \( \mathcal{L}_{\text{outside}} \) with respect to \( A_i \) is:

\begin{equation}
\frac{\partial \mathcal{L}_{\text{outside}}}{\partial A_i} = -\frac{1}{|\mathcal{S}|} \ln \left( \frac{A_i}{A_{j^*}} \right),
\end{equation}

where \( j^* \) is the index in \( \mathcal{O} \) that maximizes \( D_{\text{sym}}(A_i, A_j) \). This gradient pushes \( A_i \) away from \( A_{j^*} \), enhancing distinction between object tokens and outside tokens.

\textbf{Gradient of PAC-Bayes Regularizer}

The gradient of the PAC-Bayes regularizer \( \mathcal{R}_{\text{PAC}} \) with respect to \( A_{\text{object}k} \) is:

\begin{equation}
\frac{\partial \mathcal{R}_{\text{PAC}}}{\partial A_{\text{object}k}} = \frac{1}{4N \mathcal{R}_{\text{PAC}}} \ln \left( \frac{A_{\text{object}k}}{U} \right).
\end{equation}

This gradient penalizes deviations from the uniform distribution, preventing overfitting.



\newpage

\section{Experiment}

CLIP Score based on the Attend and Excite Dataset [TBD]].

\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
Method & \multicolumn{3}{c|}{Animal-Animal} & \multicolumn{3}{c|}{Animal-Object} & \multicolumn{3}{c|}{Object-Object} \\
\hline
 & Full Sim. & Min. Sim. & T-C Sim. & Full Sim. & Min. Sim. & T-C Sim. & Full Sim. & Min. Sim. & T-C Sim. \\
\hline
SD [TBD] & 0.311 & 0.213 & 0.767 & 0.340 & 0.246 & 0.793 & 0.335 & 0.235 & 0.765 \\
CD [TBD] & 0.284 & 0.232 & 0.692 & 0.336 & 0.252 & 0.769 & 0.349 & 0.265 & 0.759 \\
StrD [TBD] & 0.306 & 0.210 & 0.761 & 0.336 & 0.242 & 0.781 & 0.332 & 0.234 & 0.762 \\
EBCA [TBD] & 0.291 & 0.215 & 0.722 & 0.317 & 0.229 & 0.732 & 0.321 & 0.231 & 0.726 \\
AnE [TBD] & 0.332 & 0.248 & 0.806 & 0.353 & 0.265 & 0.830 & 0.360 & 0.270 & 0.811 \\
SG [TBD] & 0.311 & 0.213 & 0.767 & 0.355 & 0.264 & 0.830 & 0.355 & 0.262 & 0.811 \\
EBAMA [TBD] & 0.340 & 0.256 & 0.817 & 0.362 & 0.270 & 0.851 & 0.366 & 0.274 & 0.836 \\
D\&B [TBD] & 0.331 & 0.246 & 0.81 & -- & -- & -- & -- & -- & -- \\
\hline
Ours & 0.348 & 0.262 & 0.823 & -- & -- & -- & -- & -- & -- \\

\hline
\end{tabular}


\section{Algorithm}

\begin{algorithm}[H]
\caption{A Single Denoising Step using PAC}
\label{alg:syngen_step}
\begin{algorithmic}[1]
\Statex \textbf{Input:} Text prompt $P$, latents $\mathbf{z}_t$, text embeddings $\mathbf{E}$, timestep $t$, iteration $i$, step size $\alpha_t$, number of intervention steps $K$, trained Stable Diffusion model $\text{SD}$, loss hyperparameters $\lambda_{\text{div}}$, $\lambda_{\text{sim}}$, $\lambda_{\text{out}}$, $\lambda_{\text{PAC}}$
\Statex \textbf{Output:} Updated latents $\mathbf{z}_t$
\State $\mathbf{z}_t \gets \mathbf{z}_t.\operatorname{detach}().\operatorname{requires\_grad\_}(True)$
\For{each latent $\mathbf{z}_t^{(n)}$ and text embedding $\mathbf{E}^{(n)}$}
    \State Reset gradients
    \State Compute noise prediction and attention maps: \par
    \hskip\algorithmicindent $(\boldsymbol{\epsilon}_\theta, \mathbf{A}_t) \gets \text{SD}(\mathbf{z}_t^{(n)}, P, t, \mathbf{E}^{(n)})$
    \State Aggregate attention maps: \par
    \hskip\algorithmicindent $\{\mathbf{A}_i\} \gets \operatorname{AggregateAttentionMaps}(\mathbf{A}_t)$
    \State Compute total loss: \par
    \hskip\algorithmicindent $\mathcal{L} = \lambda_{\text{div}} \mathcal{L}_{\text{div}} + \lambda_{\text{sim}} \mathcal{L}_{\text{sim}} + \lambda_{\text{out}} \mathcal{L}_{\text{out}} + \lambda_{\text{PAC}} \mathcal{R}_{\text{PAC}}$
    \If{$i < K$}
        \State Update latent: $\mathbf{z}_t^{(n)} \gets \mathbf{z}_t^{(n)} - \alpha_t \nabla_{\mathbf{z}_t^{(n)}} \mathcal{L}$
    \EndIf
\EndFor
\State \textbf{Return} $\mathbf{z}_t$
\end{algorithmic}
\end{algorithm}


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
